Easy Variational Inference for Categorical Models via an Independent Binary Approximation

We pursue tractable Bayesian analysis of generalized linear models (GLMs) for categorical data. Thus far, GLMs are difficult to scale to more than a few dozen categories due to non-conjugacy or strong posterior dependencies when using conjugate auxiliary variable methods. We define a new class of GLMs for categorical data called categorical-from-binary (CB) models. Each CB model has a likelihood that is bounded by the product of binary likelihoods, suggesting a natural posterior approximation. This approximation makes inference straightforward and fast; using well-known auxiliary variables for probit or logistic regression, the product of binary models admits conjugate closed-form variational inference that is embarrassingly parallel across categories and invariant to category ordering. Moreover, an independent binary model simultaneously approximates multiple CB models. Bayesian model averaging over these can improve the quality of the approximation for any given dataset. We show that our approach scales to thousands of categories, outperforming posterior estimation competitors like Automatic Differentiation Variational Inference (ADVI) and No U-Turn Sampling (NUTS) in the time required to achieve fixed prediction quality.

==> app_vi_for_hier_sdo.tex <==

\subsection{Variational family}
We take the mean-field variational family for the Hierarchical SDO-probit model  \eqref{eqn:HDOP} to have density given by
{\footnotesize 
	\begin{align*}
	& q(\+z, \+\beta,  \+\mu,   \+\Sigma) \stackrel{1}{=}   q(\+\beta) q(\+z) q(\+\Sigma)  q(\+\mu)  \\
	& \stackrel{2}{=}  \ds\prod_{k=1}^K \explaintermbrace{$\N (\qm_k, \qV_k)$ \; }{q(\+\mu_k)}  \explaintermbrace{\; $\InverseWishart (\qnu_k, \qS_k)$ \;}{q(\+\Sigma_k)} \ds\prod_{j=1}^J  \explaintermbrace{$\N(\qmu_{jk},  \qSigma_{jk})$\; }{q(\+\beta_{jk})}  \ds\prod_{i=1}^{N_j} \explaintermbrace{\; $\TruncatedNormal (\wt{\eta}_{ijk},  1,  \Omega_{ijk})$}{q(z_{ijk})} 
	\labelit \label{eqn:mf_variational_family_for_hierarchical_DO_probit}
	\\ & \text{where} \; \Omega_{ijk} = 
	\begin{cases}
	\R^+, & y_{ij} = k \\
	\R^-, & \text{otherwise} \\
	\end{cases}
	\labelit \label{eqn:trunation_region_for_aux_var_in_H_SDO}
	\end{align*}
}Equality (1) is by mean-field assumption,  and,  as we see below,  (2) is the optimal such form as per \algorithm. %(2) falls out automatically from \eqref{eqn:DO_probit_lower_bound},  since the optimal mean-field coordinate updates (with respect to the traditional ELBO) are proportional to the exponentiated expected log joint density (\cite{blei2017variational}), and (3) gives the specific forms for the optimal densities using the complete conditionals in Section \ref{sec:HDOP_surrogate_ccs},  and the fact that optimal variational updates (with respect to the traditional ELBO) all belong to the same subfamilies as the complete conditionals when those complete conditionals belong to the exponential family (\cite{blei2017variational}).    Note that we use the tilde to designate \textit{variational} parameters.   

%and where $\TruncatedNormal$ denotes the univariate truncated normal distribution defined in Section \ref{sec:DOP_model}.   

\subsection{Surrogate complete conditionals} \label{sec:HDOP_surrogate_ccs}
The hierarchical Bayesian DO-Probit model \eqref{eqn:HDOP} has a surrogate model which is a hierarchical Bayesian linear regression on the auxilliary variables $\+z$.   In this way,  we obtain the surrogate complete conditionals
{\footnotesize
\begin{align*}
z_{ijk} \cond \+\beta_{j1}, ..., \+\beta_{jK},  y_{ij} & \sim 
\begin{cases}
\N_+ \bigg(  \+x_{ij}^T \+\beta_{jk} \; , \; 1 \bigg), & y_{ij} = k \\
\N_- \bigg( \+x_{ij}^T \+\beta_{jk} \; ,  \; 1 \bigg),  & \text{otherwise} 
\end{cases}  
\labelit \label{eqn:cc_for_zi_hierarchical_DO_probit} 
\end{align*}
where $\N_+$ and $\N_-$ are truncated normal distributions defined in Section \ref{sec:normal_plus_and_normal_minus}, and
\begin{align*}
&\+\beta_{jk} \cond \+z_{jk},   \+\mu_k,  \+\Sigma_k  \sim \N (\+\mu_{jk}^\prime,  \+\Sigma_{jk}^\prime), \\
& \+\mu_{jk}^\prime  = \+\Sigma_{jk}^\prime  \bigg( \+\Sigma_k^{-1} \+\mu_k + \+X_j^T \+z_{jk} \bigg),  \quad
\+\Sigma_{jk}^\prime = \bigg( \+\Sigma_k^{-1} + \+X_j^T \+X_j \bigg)^{-1}
\labelit \label{eqn:cc_for_beta_hierarchical_DO_probit} 
\end{align*}
and
\begin{align*}
\+\Sigma_k &\cond \+\mu_k,  \+\beta_{1k},  ..., \+\beta_{Jk}  \sim \InverseWishart \bigg( \nu_0 + J,   \+S_0 + \+S_{\+\mu_k}  \bigg), \\
 \+S_{\+\mu_k} & := \ds\sum_{j=1}^J (\+\beta_{jk} - \+\mu_k)   (\+\beta_{jk} - \+\mu_k)^T 
 \labelit \label{eqn:cc_for_Sigma_hierarchical_DO_probit} 
\end{align*}
and
\begin{align*}
\+\mu_k &\cond \+\Sigma_k,  \+\beta_{1k},  ..., \+\beta_{Jk}  \sim \N (\+m_k^\prime,  \+V_k^\prime), \\
 \+m_k^\prime  &= \+V_k^\prime \bigg(\+V_0 \+m_0 + J \+\Sigma_k^{-1} \overline{\+\beta_k} \bigg),  \quad \quad \overline{\+\beta_k}  := \df{1}{J} \ds\sum_{j=1}^J \+\beta_{jk} \\
 \+V_k^\prime  &= \bigg(  \+V_0^{-1} + J \+\Sigma_k^{-1} \bigg)^{-1} 
 \labelit \label{eqn:cc_for_mu_hierarchical_DO_probit} 
\end{align*}
}
%\red{Keep this?} Note in (1) and (2) that there is no scalar variance term preceding $\+X_{j}^T \+z_{jk}$ or $\+X_j^T \+X_j$, respectively,  since the model fixes the variance of the latent variables $z_{ijk}$ to 1.


\subsection{Coordinate ascent updates}

All of the surrogate complete conditionals are in the exponential family,  and hence  we know from  \algorithm \, that the optimal variational factors with respect to the surrogate lower bound $\L_\HSDOP$ are in the same exponential family,  with parameters given by  \eqref{eqn:optimal_CAVI_for_EFCC}.  Here we derive the parameters for the updates,  using the notation of \eqref{eqn:mf_variational_family_for_hierarchical_DO_probit}.


% Hence,  the formalism for handling exponential family complete conditionals \eqref{eqn:optimal_CAVI_for_EFCC}
  
 
\paragraph{Updates to $ \{q(\+\beta_{jk}) \}_{jk}$} Since the natural parameters of a multivariate Gaussian are the precision and precision-weighted mean,  we reparametrize the surrogate complete conditional for each $\+\beta_{jk}$ in \eqref{eqn:cc_for_beta_hierarchical_DO_probit} before taking variational expectations of the parameters.   Hence,   the optimal update to each $q(\+\beta_{jk} \cond \qmu_{jk},  \qSigma_{jk})$ with respect to the objective $\L_\HSDOP$ is given by
{\footnotesize
 \begin{align*}
\qSigma_{jk}^{-1} &=  \E_{q_{-\+\beta_{jk}}} \bigg[  \+\Sigma_k^{-1} + \+X_j^T \+X_j \bigg]   =  \E_{q_{\+\Sigma_k}} [ \+\Sigma_k^{-1}] +  \+X^T_j \+X_j \\
& \stackrel{1}{=}  \qS_k^{-1} \qnu_k +  \+X^T_j \+X_j \\
\qSigma_{jk}^{-1} \qmu_{jk} &=  \E_{q_{-\+\beta_{jk}}} \bigg[  \+\Sigma_k^{-1} \+\mu_k + \+X_j^T  \+z_{jk} \bigg]  \\
&=  \E_{q_{\+\Sigma_k}} [ \+\Sigma_k^{-1}] \E_{q_{\+\mu_k}} [ \+\mu_k] +  \+X^T_j  \E_{q_{\+z_{jk}}}[ \+z_{jk}] \\
& \stackrel{2}{=}  \qnu_k \qS_k^{-1} \qm_k +  \+X_j^T  \E_{q_{\+z_{jk}}}[ \+z_{jk}]  
 \end{align*}
 }where $\E_q[\+z_{jk}]$ is given explicitly below.   Equations (1),  (2) follow from Sec. \ref{sec:inverse_wishart_distribution}.


Thus,  in standard parameterization, we update
{\footnotesize
 \begin{align*}
 \qmu_{jk} &= \qSigma_{jk} \bigg(   \qnu_k \qS_k^{-1} \qm_k +  \+X_j^T  \E_{q_{\+z_{jk}}}[ \+z_{jk}] \bigg)  \\
\qSigma_{jk} &=  \bigg( \qS_k^{-1} \qnu_k +  \+X^T_j \+X_j  \bigg)^{-1}
 \end{align*}
}where $\E_q[\+z_{jk}]   \in \R^{N_j}$ has $i$-th entry given by 
{\footnotesize
\begin{align*}
\E_q[z_{ijk}] = 
\begin{cases}
\wt{\eta}_{ijk} + \df{\phi{(-\wt{\eta}_{ijk})}}{1 - \Phi{(-\wt{\eta}_{ijk})}},& y_{ij} = k\\
\wt{\eta}_{ijk} - \df{\phi{(-\wt{\eta}_{ijk})}}{\Phi(-\wt{\eta}_{ijk})}, & \text{otherwise} 
\end{cases} 
\end{align*} 
}by properties of the truncated normal distribution (Section \ref{sec:normal_plus_and_normal_minus}).   Recall that $\phi$ and $\Phi$ refer to the pdf and cdf,  respectively,  of the standard normal. 


\paragraph{Updates to $ \set{q(\+\mu_k)}_k$} Since the natural parameters of a multivariate Gaussian are the precision and precision-weighted mean,  we reparametrize the surrogate complete conditionals for $\+\mu_k$ in \eqref{eqn:cc_for_mu_hierarchical_DO_probit} before taking variational expectations of the parameters.  Hence,  the optimal update to $q(\+\mu_k \cond \qm_k,   \qV_k)$ with respect to the objective $\L_\HSDOP$ is given by 
{\footnotesize
  \begin{align*}
\qV_k^{-1} &=  \E_{q_{-\+\mu+k}} \bigg[  \+V_0^{-1} + J \+\Sigma_k^{-1} \bigg]  = \+V_0^{-1} + J   \, \E_{q_{\+\Sigma_k}} [ \+\Sigma_k^{-1} ] \\
&\stackrel{1}{=}  \+V_0^{-1} + J \qS_k^{-1} \qnu_k \\
\qV_k^{-1} \qm_k &=  \E_{q_{-\+\mu_k}} \bigg[  \+V_0^{-1} \+m_0 + J \+\Sigma_k^{-1}   \sum_{j=1}^J \+\beta_{jk}  \bigg] \\
& =  \+V_0^{-1} \+m_0 + \cancel{J}  \, \E_{q_{\+\Sigma_k}} [ \+\Sigma_k^{-1} ] \, \cancel{\frac{1}{J}} \ds\sum_{j=1}^J \E_{q_{\+\beta_{jk}}} [\+\beta_{jk}] \\
& \stackrel{2}{=}  \+V_0^{-1} \+m_0 +  \qS_k^{-1} \qnu_k \,  \ds\sum_{j=1}^J \qmu_{jk}
 \end{align*} 
}Equations (1),  (2) follow from Sec. \ref{sec:inverse_wishart_distribution}.
 
Thus,  in standard parameterization,  we update
{\footnotesize
 \begin{align*}
 \qm_k = \qV_k \bigg(   \+V_0^{-1} \+m_0 +  \qS_k^{-1} \qnu_k \,  \ds\sum_{j=1}^J \qmu_{jk}  \bigg),  \quad
\qV_k =  \bigg(    \+V_0^{-1} + J \qS_k^{-1} \qnu_k \bigg)^{-1}
 \end{align*}
 }
 
\paragraph{Updates to $ \set{q(\+\Sigma_k)}_k$} Since the natural parameters of an Inverse Wishart are identical to the conventional parameters (up to a multiplicative scalar constant),  we do not need to reparametrize the surrogate complete conditional for $\+\Sigma_k$ in \eqref{eqn:cc_for_Sigma_hierarchical_DO_probit}  before taking variational expectations of the parameters.   Hence,  the optimal update to $q(\+\Sigma_k \cond \qS_k, \qnu_k)$ with respect to the objective $\L_\HSDOP$ is given by
 {\footnotesize
 \begin{align*}
\qnu_k  &=  \E_{q_{-\+\Sigma}}  \bb{ \nu_0 + J }   =  \nu_0 + J \\
\qS_k &= \E_{q_{-\+\Sigma}}  \bb{\+S_0 + \ds\sum_{j=1}^J  (\+\beta_{jk} - \+\mu_k) (\+\beta_{jk} - \+\mu_k)^T }  \\
&= \+S_0 + \ds\sum_{j=1}^J  \E_{q_{-\+\Sigma}}  \bb{\+\beta_{jk}  \+\beta_{jk}^T  -  \+\beta_{jk}\+\mu_k^T  +\+\mu_k \+\beta_{jk}^T + \+\mu_k \+\mu_k^T } \\
& \stackrel{(+)}{=} \+S_0 +  J\qV_k + \ds\sum_{j=1}^J \qSigma_{jk} + (\qmu_{jk} - \qm_k)(\qmu_{jk} - \qm_k)^T
 \labelit \label{eqn:update_to_psi_for_bayesian_hierarchical_regression}
 \end{align*}
} where in (+) we used
{\footnotesize \begin{align*}
\E_q [ \+\mu_k  \+\mu_k^T] &= \Var_q[\+\mu_k  ] + \E_q [ \+\mu_k   ]  \E_q [ \+\mu_k  ]^T= \qV_k + \qm_k \qm_k^T \\
\E_q [ \+\beta_{jk}\+\beta_{jk}^T] &=  \Var_q[\+\beta_{jk}] + \E_q [ \+\beta_{jk}]  \E_q [\+\beta_{jk}]^T = \qSigma_{jk} + \qmu_{jk} \qmu_{jk}^T \\
\intertext{and}
\E_q [ \+\beta_{jk} \+\mu_k  ^T] & \stackrel{\text{(mean field)}}{=} \E_q[ \+\beta_{jk}] \E_q[ \+\mu _k ^T] = \qmu_{jk} \qm_k^T
 \end{align*}
}with $\E_q [\+\mu_k \+\beta_{jk}^T]$ handled similarly as $\E_q [ \+\beta_{jk}  \+\mu_k  ^T] $.


\paragraph{Updates to $ \set{q(z_{ijk})}_{ijk}$}

In \eqref{eqn:cc_for_zi_hierarchical_DO_probit} ,  we saw that the surrogate complete conditional for each $z_{ijk}$ has the form $\TruncatedNormal(\eta_{ijk}, 1, \Omega_{ijk})$,  where $\Omega_{ijk}$ is defined as in \eqref{eqn:trunation_region_for_aux_var_in_H_SDO}. But since each such distribution is in the exponential family with natural parameter $\eta_{ijk}$,  the optimal update for each $q(z_{ijk})$ is given by
{\footnotesize
\begin{align*}
\qeta_{ijk} =\E[\+x_{ij}^T \+\beta_{jk}] = \+x_{ij}^T \qmu_{jk} 
\end{align*} 
}

\subsection{Lower bound} \label{sec:surrogate_lower_bound_hierarchical_DO_probit}

%Our tractable surrogate lower bound on the marginal log likelihood,  $\L_\HSDOP$,  is provided explicitly in Appendix \ref{sec:surrogate_lower_bound_hierarchical_DO_probit_APPENDIX}. 

%\subsection{Lower bound on the log marginal likelihood for the Hierarchical DO-Probit} \label{sec:surrogate_lower_bound_hierarchical_DO_probit_APPENDIX}


A tractable surrogate lower bound on the marginal log likelihood for the Hierarchical DO-Probit model \eqref{eqn:HDOP} -- useful for tracking the monotonic increase in the objective function and  setting a convergence criterion -- can immediately be obtained by handling the expected complete data likelihood precisely as in Section \ref{sec:lower_bound_for_DOP}
{ \scriptsize
	\begin{align*}
	& \ELBO_\HSDOP(q; \+y)  =  \explaintermbrace{energy}{\E_q [\log p_\HSDOP(\+y,  \+z, \+\beta, \+\mu, \+\Sigma)]}  \explaintermbrace{entropy}{- \E_q [\log q (\+z,  \+\beta, \+\mu,  \+\Sigma )]}\\
	 &= \E_q [\log p_\SDO(\+y,  \+z \cond \+\beta)]+ \H[q(\+z)] - \KL{q(\+\beta, \+\mu, \+\Sigma)}{p  (\+\beta,  \+\mu, \+\Sigma)}  \\
	 & \stackrel{\eqref{eqn:expected_cdl_of_sdo_probit_dominates}}{\geq}   \E_q [\log p_\IBP(\wb{\+y},  \+z \cond \+\beta)]  + \H[q(\+z)] - \KL{q(\+\beta, \+\mu, \+\Sigma)}{p (\+\beta,  \+\mu, \+\Sigma)}  \\
	 & = \ELBO_\IBP(q, \wb{\+y}) - \KL{q( \+\mu, \+\Sigma)}{p (\+\mu, \+\Sigma)}  := \L_\HSDOP(q; \+y) 
	 \labelit \label{eqn:HDO_probit_lower_bound}
	\end{align*} 
}We expand this lower bound using:
{ \footnotesize
	\begin{align*}
	& \mathcal{L}_\HSDOP(q)  =  \ds\sum_{j=1}^J \ds\sum_{i=1}^{N_j}  \ds\sum_{k=1}^K \explaintermbrace{(A)}{\E_q [\log p_\IBP(\wb{y}_{ijk},  z_{ijk} \cond \+\beta_{jk}) ]} \\
	& \quad + \ds\sum_{j=1}^J \ds\sum_{i=1}^{N_j}  \ds\sum_{k=1}^K \explaintermbrace{(B)}{ \H [ q(z_{ijk})]} + \; \ds\sum_{k=1}^K  - \explaintermbrace{(C)}{\KL{q(\+\mu_k)}{p_\HSDOP(\+\mu_k)}} \;  \\
	& \quad  + \ds\sum_{k=1}^K - \explaintermbrace{(D)}{\KL{q(\+\Sigma_k)}{p_\HSDOP(\+\Sigma_k)}} \\
	& \quad +\ds\sum_{j=1}^J \ds\sum_{k=1}^K -  \explaintermbrace{(E)}{\E_q \bigg[ \KL{q(\+\beta_{jk})}{p_\HSDOP(\+\beta_{jk} \cond \+\mu_k,  \+\Sigma_k)} \bigg]}.
	\end{align*}
}

In particular term (A) is given by
	\begin{align*}
	 & \E_q [\log p_\IBP(\wb{y}_{ijk},  z_{ijk} \cond \+\beta_{jk}) ]  \\
	 & \quad =   -\half ( \log 2\pi +1 ) +  \half \wt{\eta}_{ijk} \delta_{\wb{y}_{ijk}} (\wt{\eta}_{ijk}) -\half \+x_{ij}^T \wt{\+\Sigma}_k \+x_{ij} 
	\end{align*} 
where
	\begin{align*}	
	\wt{\eta}_{ijk}= \+x_{ij}^T \wt{\+\mu}_k  \quad  \text{and} \quad 	\delta_{b} (x) :=
	\begin{cases}
	\df{\phi(-x)}{1 - \Phi(-x)} ,  & b = 1\\
	- \df{\phi(-x)}{\Phi(-x)} ,  & b  = 0
	\end{cases}
	\end{align*} 

Term (B) is the entropy of a truncated normal distribution,  where the $(ijk)$-th element in the sum is

\begin{itemize}
 \item  the entropy of $\N_+(\+x_{ij}^T \wt{\+\mu}_k,  1)$ when $y_{ij}=k$,   in which case the entropy is given by \eqref{eqn:entropy_of_normal_plus} 
 \item the entropy of  $\N_-(\+x_{ij}^T \wt{\+\mu}_k,  1)$ when $y_{ij} \neq k$,  in which case the entropy is given by  \eqref{eqn:entropy_of_normal_minus}.  
 \end{itemize}
 
Term C is the KL divergence between two multivariate Gaussians; in this case we have
{ \scriptsize
	\begin{align*}	 
	&\KL{q(\+\mu_k)}{p(\+\mu_k)} \\\
	&\; = -\half \bigg[   \log \df{|\+V_0|}{|\wt{\+V}_k|} - M + (\wt{\+m}_k - \+m_0)^T \+V_0^{-1} (\wt{\+m}_k - \+m_0) + \tr (\+V_0^{-1} \wt{\+V}_k) \bigg] 
	\end{align*} 
}

Term D is the KL divergence between two Inverse Wisharts;  in this case,  we have
{ \footnotesize
	\begin{align*}	
	&\KL{q(\+\Sigma_k)}{p(\+\Sigma_k)} = \log  \bigg(\df{\Gamma_M(\frac{\nu_0}{2})}{\Gamma_M(\frac{\wt{\nu}_k}{2})} \bigg) + \df{\wt{\nu}_k}{2} \tr (\wt{\+S}_k^{-1} \+S_0) \\
	&\quad - \df{ \wt{\nu}_k M}{2} - \df{\nu_0}{2} \log |\wt{\+S}_k^{-1} \+S_0 | - \df{\nu_0 - \wt{\nu}_k}{2} \ds\sum_{i=1}^M \psi \bigg(\df{\wt{\nu}_k - M + i}{2} \bigg)
		\end{align*} 
}where $\Gamma_M$ is the multivariate gamma function and $\psi$ is the digamma function given by $\psi(x) := \frac{d}{dx} \ln \Gamma_1(x)$. 

Term E gives the expected KL divergence between two multivariate Gaussians,  in the specific case where the expectation is taken with respect to independent Gaussian and Inverse Wishart distributions on the parameters of the second argument of the KL divergence.   Utilizing the mean-field assumption, we find
{ \footnotesize 
	\begin{align*}
	& \E_{q(\+\mu_k \cond \wt{\+m}_k,  \wt{\+V}_k)  q(\+\Sigma_k \cond \wt{\nu}_k,  \wt{\+S}_k)} \bigg[ \KL{q(\+\beta_{jk} \cond \wt{\+\mu}_{jk},  \wt{\+\Sigma}_{jk}) }{p(\+\beta_{jk} \cond \+\mu_k,  \+\Sigma_k)}  \bigg] \\
	&= \half \Bigg[ -M \,  (\log 2 +1) + \log |\wt{\+S}_k | - \ds\sum_{i=1}^M \psi \bigg( \df{\wt{\nu}_k - i + 1}{2} \bigg)  - \log | \wt{\+\Sigma}_{jk} | \\
	&+ \tr \bigg(\wt{\nu}_k \wt{\+\Psi}_k^{-1} \big[  \wt{\+\mu}_{jk}  \wt{\+\mu}_{jk}^T - \wt{\+\mu}_{jk}  \wt{\+m}_k^T - \wt{\+m}_k \wt{\+\mu}_{jk}^T +  \wt{\+V}_k + \wt{\+m}_k \wt{\+m}_k^T +  \wt{\+\Sigma}_{jk} \big] \bigg)  \Bigg]. 
	\end{align*}
	}

%\wt{\+S}
%\wt{\nu}
%where the $\wb{y}_{ik}$ refers to the one-versus-rest labeling scheme of \eqref{eqn:binary_regression_labels_for_identified_DO_probit}.  Equality (1) uses the same argument as in Section \ref{sec:lower_bound_for_DO_Probit}.


==> fig_IB_for_categorical_predictions.tex <==
\begin{figure*}
\begin{tabular}{c c}
\raisebox{-.5\height}{
\includegraphics[width=0.36\textwidth]{images/proba_posterior_visualization_IB_K3_N16_and_N1024.pdf}
}
&
\begin{tabular}{r r r | r r r }					
N	& IB + DO 	& IB + SDO	& SDO 	    & DO	        & Cat. MLE
\\		
\midrule
2	&-1.6923	&-0.9221	&-0.9754		&-0.8869		&-5.6252
\\
16	&-1.3300	&-0.7045	&-0.7251		&-0.6958		&-5.5333
\\
128	&-1.3089	&-0.6902	&-0.6908		&-0.6907		&-0.6970
\\
1024&-1.3067	&-0.6885	&-0.6885		&-0.6885		&-0.6886
\\
8192&-1.3070	&-0.6887	&-0.6887		&-0.6887		&-0.6887
\end{tabular}
\end{tabular}
\caption{Comparison of categorical predictions using posterior samples from the IB binary model. In this intercept-only (no covariates) setting, we find that IB + SDO offers indistinguishable performance from (harder-to-fit, non-conjugate) categorical models, and
superior performance to the IB+DO alternative.
IB generates binary vectors by design and thus requires a post-hoc estimator (denoted ``+DO'' or ``+SDO''; defined in Sec.~\ref{sec:IB_estimators}) to ensure valid categorical predictions.
\emph{Left:}
Visualization of posterior over the probability of category 2, whose true frequency is 0.7.
\emph{Right:}
Average log likelihood on heldout set for each model as size of training set $N$ increases. 
For most methods, we compute the predictive likelihood $\log p( y_* | y_{1:N})$, marginalizing out weights via Monte Carlo averages of posterior samples.
Cat MLE baseline just point estimates category frequencies via maximize likelihood.
\emph{Setting:}
We fit to the first $N$ examples of a toy dataset, generated with $K=3$ categories with ground truth frequencies [0.02, 0.7, 0.28].
All models use a standard Normal prior over weights.
}%endcaption
\label{fig:IB_for_categorical_predictions}
\end{figure*}
%\begin{tabular}{rrr}
%\toprule
%   N &        DO &       MLE \\
%\midrule
%   2 & -0.886948 & -5.625216 \\
%  16 & -0.695786 & -5.533336 \\
% 128 & -0.690665 & -0.697006 \\
%1024 & -0.688539 & -0.688628 \\
%8192 & -0.688677 & -0.688688 \\
%\bottomrule
%\end{tabular}
%\begin{tabular}{rrr}
%\toprule
%   N &       DO &       SDO \\
%\midrule
%   2 & -1.69226 & -0.922148 \\
%  16 & -1.32999 & -0.704454 \\
% 128 & -1.30888 & -0.690221 \\
%1024 & -1.30669 & -0.688503 \\
%8192 & -1.30697 & -0.688671 \\
%\bottomrule
%\end{tabular}
%\begin{tabular}{rr}
%\toprule
%   N &       SDO \\
%\midrule
%   2 & -0.975392 \\
%  16 & -0.725111 \\
% 128 & -0.690806 \\
%1024 & -0.688497 \\
%8192 & -0.688662 \\
%\bottomrule
%\end{tabular}


==> fig_visualize_DO_vs_IB.tex <==
\begin{figure}[!t]
\setlength{\tabcolsep}{0.01cm}  %% space between columns
\begin{tabular}{c c c}
{\includegraphics[width=0.16\textwidth]{images/beta_posterior_visualization_DO_K3_N16_and_N1024.pdf}
}
&
{\includegraphics[width=0.16\textwidth]{images/beta_posterior_visualization_SDO_K3_N16_and_N1024.pdf}
}
&
{\includegraphics[width=0.16\textwidth]{images/beta_posterior_visualization_IB_K3_N16_and_N1024.pdf}
}
\end{tabular}
\caption{\textbf{Comparison of posteriors and ML point estimates for two weight coefficients ($\beta_1, \beta_2$) in \emph{intercepts-only} setting.}
\emph{Left:} DO model for categorical observations.
\emph{Center:} Simplified DO (SDO) model, also categorical.
\emph{Right:} IB model for binary observations.
All models are intercept-only (no covariates) with standard Normal priors, and are fit to the first $N$ examples of the same dataset (top row $N=16$, bottom $N=8192$), generated with $K=3$ categories with ground truth frequencies [0.02, 0.7, 0.28]. 
%For $N=16$ the ML estimator is not visible because the first category appears zero times in the first 16 observations.
}%endcaption
\label{fig:visualize_posteriors_DO_vs_IB}
\end{figure}
%\begin{tabular}{rrr}
%\toprule
%   N &        DO &       MLE \\
%\midrule
%   2 & -0.886948 & -5.625216 \\
%  16 & -0.695786 & -5.533336 \\
% 128 & -0.690665 & -0.697006 \\
%1024 & -0.688539 & -0.688628 \\
%8192 & -0.688677 & -0.688688 \\
%\bottomrule
%\end{tabular}
%\begin{tabular}{rrr}
%\toprule
%   N &       DO &       SDO \\
%\midrule
%   2 & -1.69226 & -0.922148 \\
%  16 & -1.32999 & -0.704454 \\
% 128 & -1.30888 & -0.690221 \\
%1024 & -1.30669 & -0.688503 \\
%8192 & -1.30697 & -0.688671 \\
%\bottomrule
%\end{tabular}
%\begin{tabular}{rr}
%\toprule
%   N &       SDO \\
%\midrule
%   2 & -0.975392 \\
%  16 & -0.725111 \\
% 128 & -0.690806 \\
%1024 & -0.688497 \\
%8192 & -0.688662 \\
%\bottomrule
%\end{tabular}


==> fig_visualize_DO_vs_IB_covariates.tex <==
\begin{figure}[!t]
\setlength{\tabcolsep}{0.01cm}  %% space between columns
\begin{tabular}{c c c}
{\includegraphics[width=0.16\textwidth]{images/beta_posterior_viz_with_covariates_DO_K3_N16_and_N1024.pdf}
}
&
{\includegraphics[width=0.16\textwidth]{images/beta_posterior_viz_with_covariates_SDO_K3_N16_and_N1024.pdf}
}
&
{\includegraphics[width=0.16\textwidth]{images/beta_posterior_viz_with_covariates_IB_K3_N16_and_N1024.pdf}
}
\end{tabular}
\caption{\textbf{Comparison of posteriors for two weight coefficients ($\beta_{1,2}, \beta_{3,2}$) fit to synthetic data where each example has \emph{one covariate} drawn from a standard Normal.}
\emph{Left:} DO model for categorical observations.
\emph{Center:} Simplified DO (SDO) model.
\emph{Right:} IB model for binary observations.
All models have standard Normal priors and $K=3$ categories. We fit to the first $N$ examples of the same dataset.
Unlike the intercepts-only case, IB and SDO \emph{do not} concentrate on the same weight values as $N \rightarrow \infty$.
% Each example has 1 covariate drawn from a standard Normal.
% (top row $N=16$, bottom $N=8192$), 
%Empirical class frequencies are [0.73, 0.19, 0.08] for the $K=3$ categories. 
%For $N=16$ the ML estimator is not visible because the first category appears zero times in the first 16 observations.
}%endcaption
\label{fig:visualize_posteriors_DO_vs_IB_covariates}
\end{figure}
%\begin{tabular}{rrr}
%\toprule
%   N &        DO &       MLE \\
%\midrule
%   2 & -0.886948 & -5.625216 \\
%  16 & -0.695786 & -5.533336 \\
% 128 & -0.690665 & -0.697006 \\
%1024 & -0.688539 & -0.688628 \\
%8192 & -0.688677 & -0.688688 \\
%\bottomrule
%\end{tabular}
%\begin{tabular}{rrr}
%\toprule
%   N &       DO &       SDO \\
%\midrule
%   2 & -1.69226 & -0.922148 \\
%  16 & -1.32999 & -0.704454 \\
% 128 & -1.30888 & -0.690221 \\
%1024 & -1.30669 & -0.688503 \\
%8192 & -1.30697 & -0.688671 \\
%\bottomrule
%\end{tabular}
%\begin{tabular}{rr}
%\toprule
%   N &       SDO \\
%\midrule
%   2 & -0.975392 \\
%  16 & -0.725111 \\
% 128 & -0.690806 \\
%1024 & -0.688497 \\
%8192 & -0.688662 \\
%\bottomrule
%\end{tabular}


==> inputs/autodiff_all_results.tex <==
\scriptsize
\begin{longtable}{rrrr|rllrrrr|rllrr}
\toprule
\multicolumn{4}{c|}{context} & \multicolumn{7}{|c|}{error}  & \multicolumn{5}{|c|}{time (seconds)} \\
& & & &\multicolumn{5}{|c|}{MLE} & \multicolumn{2}{|c|}{CAVI} & \multicolumn{4}{|c|}{MLE} & \multicolumn{1}{|c|}{CAVI}  \\
 K &  M &     N &  seed &   SM &         SDO &          DO &  IB+DO &  IB+SDO &  IB+DO &  IB+SDO &    SM &      SDO &      DO &    IB &  \\
\midrule
 3 &  1 &   100 &     0 & 0.17 &  0.18 &  0.15 &   0.20 &    0.17 &     0.18 &      0.16 &  2.62 &     5.72 &    9.49 &  3.70 &  0.03 \\
 3 &  1 &   100 &     1 & 0.19 &   0.2 &  0.24 &   0.37 &    0.20 &     0.35 &      0.20 &  2.57 &     5.49 &    9.03 &  2.99 &  0.02 \\
 3 &  1 &   100 &     2 & 0.16 &  0.16 &  0.16 &   0.22 &    0.16 &     0.21 &      0.15 &  2.36 &     5.14 &    8.97 &  2.75 &  0.02 \\
 3 &  1 &  1000 &     0 & 0.04 &  0.04 &  0.04 &   0.16 &    0.09 &     0.15 &      0.10 &  2.63 &      5.4 &    10.2 &  3.66 &  0.10 \\
 3 &  1 &  1000 &     1 & 0.05 &  0.06 &  0.06 &   0.16 &    0.08 &     0.15 &      0.08 &  2.54 &     5.75 &    9.64 &  3.38 &  0.11 \\
 3 &  1 &  1000 &     2 & 0.04 &  0.04 &  0.05 &   0.09 &    0.04 &     0.08 &      0.05 &  2.52 &     5.58 &    9.86 &  3.29 &  0.06 \\
 3 &  1 & 10000 &     0 & 0.01 &  0.01 &  0.01 &   0.17 &    0.07 &     0.16 &      0.07 &  2.31 &     5.56 &    9.55 &  3.74 &  0.92 \\
 3 &  1 & 10000 &     1 & 0.01 &  0.02 &  0.19 &   0.20 &    0.05 &     0.20 &      0.06 &  2.66 &     5.75 &    9.59 &  3.04 &  1.23 \\
 3 &  1 & 10000 &     2 & 1.31 &  0.01 &  0.01 &   0.07 &    0.01 &     0.06 &      0.01 &  2.25 &     4.93 &    8.89 &  3.38 &  0.53 \\
 3 &  3 &   100 &     0 & 0.18 &  0.27 &  0.25 &   0.31 &    0.16 &     0.30 &      0.16 &  2.33 &     4.93 &    8.47 &  2.70 &  0.03 \\
 3 &  3 &   100 &     1 & 0.28 &  0.29 &  0.31 &   0.41 &    0.29 &     0.40 &      0.29 &  2.26 &      5.0 &    8.54 &  2.78 &  0.02 \\
 3 &  3 &   100 &     2 & 0.26 &  0.27 &  0.26 &   0.37 &    0.26 &     0.36 &      0.25 &  2.69 &     5.72 &    8.36 &  2.45 &  0.03 \\
 3 &  3 &  1000 &     0 & 0.06 &  0.05 &  0.05 &   0.20 &    0.08 &     0.20 &      0.09 &  2.41 &     5.12 &     9.3 &  3.36 &  0.13 \\
 3 &  3 &  1000 &     1 & 0.07 &   0.1 &  0.22 &   0.27 &    0.09 &     0.27 &      0.09 &  2.38 &      5.1 &   10.08 &  2.92 &  0.12 \\
 3 &  3 &  1000 &     2 & 0.07 &  0.08 &  0.17 &   0.23 &    0.10 &     0.22 &      0.10 &  2.31 &     5.21 &    9.58 &  2.94 &  0.15 \\
 3 &  3 & 10000 &     0 & 0.02 &  0.02 &  0.16 &   0.17 &    0.07 &     0.17 &      0.07 &  2.36 &     5.29 &    9.38 &  3.21 &  1.13 \\
 3 &  3 & 10000 &     1 & 0.02 &  0.18 &  0.17 &   0.19 &    0.06 &     0.19 &      0.07 &  2.27 &     5.61 &    9.52 &  2.84 &  1.11 \\
 3 &  3 & 10000 &     2 & 0.02 &  0.02 &  0.02 &   0.13 &    0.08 &     0.13 &      0.09 &  2.11 &     5.54 &    9.36 &  2.76 &  1.09 \\
 3 &  9 &   100 &     0 & 0.36 &   NaN &   NaN &   0.45 &    0.38 &     0.41 &      0.36 &  2.42 &     5.71 &    8.89 &  2.99 &  0.05 \\
 3 &  9 &   100 &     1 & 0.23 &  0.51 &   NaN &   0.30 &    0.23 &     0.27 &      0.23 &  2.37 &     5.46 &    8.85 &  2.88 &  0.05 \\
 3 &  9 &   100 &     2 & 0.35 &  0.45 &   NaN &   0.41 &    0.35 &     0.39 &      0.35 &  2.36 &     5.67 &    9.27 &  2.88 &  0.05 \\
 3 &  9 &  1000 &     0 & 0.11 &  0.13 &  0.23 &   0.21 &    0.14 &     0.21 &      0.16 &  2.43 &     5.35 &    9.51 &  3.01 &  0.21 \\
 3 &  9 &  1000 &     1 & 0.12 &  0.14 &  0.22 &   0.20 &    0.15 &     0.19 &      0.17 &  2.79 &     5.25 &     9.2 &  2.84 &  0.23 \\
 3 &  9 &  1000 &     2 & 0.11 &  0.12 &  0.23 &   0.23 &    0.15 &     0.23 &      0.17 &  2.35 &      5.3 &    9.43 &  2.77 &  0.25 \\
 3 &  9 & 10000 &     0 & 0.02 &  0.03 &  0.21 &   0.16 &    0.11 &     0.16 &      0.14 &  2.22 &     5.23 &    9.07 &  3.03 &  1.82 \\
 3 &  9 & 10000 &     1 & 0.02 &  0.03 &  0.22 &   0.19 &    0.10 &     0.19 &      0.13 &  2.27 &     5.13 &    9.72 &  2.96 &  1.78 \\
 3 &  9 & 10000 &     2 & 0.02 &  0.03 &   0.2 &   0.12 &    0.10 &     0.13 &      0.13 &  2.15 &     5.08 &    9.14 &  2.98 &  1.80 \\
 3 & 27 &   100 &     0 & 0.71 &   NaN &   NaN &    NaN &    0.55 &     0.58 &      0.49 &  2.87 &     5.71 &    9.19 &  3.08 &  0.11 \\
 3 & 27 &   100 &     1 & 0.62 &   NaN &   NaN &    NaN &    0.52 &     0.46 &      0.40 &  2.76 &     5.84 &    9.27 &  3.00 &  0.13 \\
 3 & 27 &   100 &     2 & 0.66 &   NaN &   NaN &    NaN &    0.55 &     0.53 &      0.44 &  2.69 &     4.91 &    9.36 &  3.38 &  0.11 \\
 3 & 27 &  1000 &     0 & 0.15 &  0.21 &  0.34 &   0.25 &    0.20 &     0.24 &      0.23 &  2.65 &     5.42 &    9.77 &  3.32 &  0.34 \\
 3 & 27 &  1000 &     1 & 0.15 &  0.21 &   0.3 &   0.24 &    0.18 &     0.23 &      0.20 &  2.90 &      5.5 &    9.07 &  3.24 &  0.36 \\
 3 & 27 &  1000 &     2 & 0.12 &  0.22 &   NaN &   0.21 &    0.17 &     0.22 &      0.20 &  2.64 &     5.56 &    9.26 &  3.28 &  0.34 \\
 3 & 27 & 10000 &     0 & 0.05 &  0.06 &   0.3 &   0.17 &    0.14 &     0.18 &      0.18 &  2.56 &     5.45 &   10.12 &  3.20 &  2.68 \\
 3 & 27 & 10000 &     1 & 0.05 &  0.06 &  0.28 &   0.18 &    0.13 &     0.18 &      0.17 &  2.49 &     5.21 &    8.98 &  3.26 &  2.68 \\
 3 & 27 & 10000 &     2 & 0.05 &  0.38 &  0.27 &   0.14 &    0.14 &     0.15 &      0.17 &  2.59 &     5.32 &    8.96 &  3.17 &  2.56 \\
 9 &  1 &   100 &     0 & 0.38 &  0.39 &  0.38 &   0.45 &    0.39 &     0.41 &      0.36 &  5.64 &    33.91 &   30.18 &  6.99 &  0.13 \\
 9 &  1 &   100 &     1 & 0.28 &  0.29 &  0.34 &   0.33 &    0.28 &     0.30 &      0.27 &  6.29 &    33.33 &   30.11 &  6.62 &  0.11 \\
 9 &  1 &   100 &     2 & 0.31 &  0.38 &  0.35 &   0.33 &    0.30 &     0.30 &      0.28 &  7.46 &    35.23 &   30.44 &  6.33 &  0.13 \\
 9 &  1 &  1000 &     0 & 0.10 &   0.1 &   0.1 &   0.14 &    0.12 &     0.14 &      0.12 &  4.72 &    31.75 &   26.85 &  5.97 &  0.64 \\
 9 &  1 &  1000 &     1 & 0.09 &  0.09 &  0.09 &   0.13 &    0.12 &     0.13 &      0.12 &  5.97 &    33.63 &   26.97 &  5.51 &  0.73 \\
 9 &  1 &  1000 &     2 & 0.09 &   0.1 &   0.1 &   0.11 &    0.09 &     0.10 &      0.09 &  5.43 &    33.16 &   26.93 &  6.47 &  0.54 \\
 9 &  1 & 10000 &     0 & 0.03 &  0.03 &  0.03 &   0.09 &    0.07 &     0.09 &      0.07 &  6.15 &    37.72 &   31.15 &  8.45 &  6.42 \\
 9 &  1 & 10000 &     1 & 0.02 &  0.02 &  0.02 &   0.09 &    0.06 &     0.09 &      0.06 &  4.90 &    36.48 &   28.87 &  6.39 &  6.14 \\
 9 &  1 & 10000 &     2 & 0.02 &  0.09 &  1.31 &   0.05 &    0.03 &     0.05 &      0.03 &  4.94 &    32.51 &   27.58 &  5.94 &  4.98 \\
 9 &  3 &   100 &     0 & 0.52 &   NaN &  0.64 &   0.50 &    0.49 &     0.44 &      0.45 &  6.42 &    34.57 &   31.25 &  7.44 &  0.18 \\
 9 &  3 &   100 &     1 & 0.46 &  0.69 &  0.59 &   0.46 &    0.44 &     0.43 &      0.42 &  5.96 &    33.97 &   30.01 &  7.17 &  0.14 \\
 9 &  3 &   100 &     2 & 0.38 &  0.53 &  0.25 &   0.42 &    0.38 &     0.38 &      0.35 &  6.26 &    33.66 &   31.07 &  6.58 &  0.14 \\
 9 &  3 &  1000 &     0 & 0.12 &  0.13 &  0.14 &   0.19 &    0.14 &     0.19 &      0.14 &  5.56 &    32.68 &   26.63 &  5.82 &  0.68 \\
 9 &  3 &  1000 &     1 & 0.10 &  0.11 &  0.12 &   0.16 &    0.13 &     0.16 &      0.13 &  4.33 &    31.65 &   27.54 &  5.84 &  0.62 \\
 9 &  3 &  1000 &     2 & 0.14 &  0.15 &  0.15 &   0.18 &    0.17 &     0.18 &      0.17 &  4.66 &     30.5 &    24.4 &  5.20 &  0.68 \\
 9 &  3 & 10000 &     0 & 0.04 &  0.04 &  0.05 &   0.11 &    0.08 &     0.11 &      0.09 &  4.67 &    30.66 &   27.17 &  5.97 &  6.36 \\
 9 &  3 & 10000 &     1 & 0.04 &  0.04 &  0.04 &   0.11 &    0.08 &     0.11 &      0.08 &  4.61 &    31.46 &   25.36 &  5.85 &  7.04 \\
 9 &  3 & 10000 &     2 & 0.04 &  0.04 &  0.04 &   0.12 &    0.09 &     0.13 &      0.10 &  5.01 &     32.9 &    25.8 &  5.69 &  7.89 \\
 9 &  9 &   100 &     0 & 0.66 &   NaN &   NaN &   0.64 &    0.64 &     0.59 &      0.60 &  5.82 &    32.89 &   28.19 &  6.78 &  0.24 \\
 9 &  9 &   100 &     1 & 0.68 &   NaN &   NaN &   0.67 &    0.64 &     0.54 &      0.55 &  5.71 &    32.52 &   28.03 &  6.30 &  0.32 \\
 9 &  9 &   100 &     2 & 0.65 &   NaN &   NaN &   0.62 &    0.63 &     0.56 &      0.58 &  5.81 &    32.21 &   28.68 &  6.23 &  0.26 \\
 9 &  9 &  1000 &     0 & 0.21 &   0.2 &  0.28 &   0.26 &    0.25 &     0.26 &      0.25 &  4.40 &    30.73 &   24.74 &  5.34 &  1.14 \\
 9 &  9 &  1000 &     1 & 0.20 &  0.24 &   0.3 &   0.27 &    0.24 &     0.26 &      0.25 &  6.06 &    30.95 &   24.64 &  5.36 &  1.22 \\
 9 &  9 &  1000 &     2 & 0.22 &  0.23 &  0.29 &   0.28 &    0.26 &     0.28 &      0.27 &  4.39 &    30.87 &   24.59 &  5.60 &  1.19 \\
 9 &  9 & 10000 &     0 & 0.06 &  0.59 &  0.25 &   0.14 &    0.15 &     0.15 &      0.16 &  4.88 &    32.85 &    25.9 &  6.23 &  9.40 \\
 9 &  9 & 10000 &     1 & 0.45 &  0.07 &  0.27 &   0.38 &    0.38 &     0.15 &      0.16 &  6.47 &    35.77 &   28.24 &  6.17 &  8.99 \\
 9 &  9 & 10000 &     2 & 0.11 &  0.44 &  0.27 &   0.15 &    0.14 &     0.15 &      0.15 &  6.43 &    32.47 &   27.76 &  6.64 &  9.52 \\
 9 & 27 &   100 &     0 &  NaN &     s &     s &    NaN &    1.21 &     0.98 &      0.91 &  6.24 &        s &       s &  7.32 &  0.71 \\
 9 & 27 &   100 &     1 & 1.24 &     s &     s &    NaN &    1.25 &     0.98 &      0.90 &  6.14 &        s &       s &  6.85 &  0.77 \\
 9 & 27 &   100 &     2 & 1.35 &     s &     s &    NaN &    1.31 &     1.04 &      0.94 &  6.11 &        s &       s &  6.82 &  0.72 \\
 9 & 27 &  1000 &     0 & 0.34 &     s &     s &   0.37 &    0.39 &     0.36 &      0.40 &  4.82 &        s &       s &  5.75 &  2.09 \\
 9 & 27 &  1000 &     1 & 0.34 &     s &     s &   0.38 &    0.39 &     0.38 &      0.40 &  4.85 &        s &       s &  5.70 &  2.14 \\
 9 & 27 &  1000 &     2 & 0.33 &     s &     s &   0.34 &    0.38 &     0.33 &      0.38 &  4.90 &        s &       s &  5.63 &  1.97 \\
 9 & 27 & 10000 &     0 & 0.34 &     s &     s &   1.02 &    0.94 &     0.17 &      0.21 &  5.13 &        s &       s &  6.37 & 15.58 \\
 9 & 27 & 10000 &     1 & 0.15 &     s &     s &   0.66 &    0.69 &     0.18 &      0.21 &  5.15 &        s &       s &  9.45 & 14.77 \\
 9 & 27 & 10000 &     2 & 0.44 &     s &     s &   1.02 &    0.96 &     0.18 &      0.21 &  5.08 &        s &       s &  6.36 & 14.45 \\
27 &  1 &   100 &     0 & 0.54 &  0.58 &  0.75 &   0.54 &    0.51 &     0.41 &      0.41 & 21.62 &  1251.51 &  106.28 & 17.57 &  0.85 \\
27 &  1 &   100 &     1 & 0.57 &  0.68 &   NaN &   0.55 &    0.54 &     0.44 &      0.43 & 19.12 &  1252.08 &  105.63 & 19.91 &  0.86 \\
27 &  1 &   100 &     2 & 0.62 &  0.75 &   NaN &   0.61 &    0.59 &     0.51 &      0.49 & 20.75 &  1277.38 &  105.41 & 22.40 &  0.83 \\
27 &  1 &  1000 &     0 & 0.18 &  0.21 &  0.24 &   0.19 &    0.18 &     0.18 &      0.18 & 17.69 &   1330.1 &  107.05 & 19.37 &  4.86 \\
27 &  1 &  1000 &     1 & 0.20 &  0.18 &  0.26 &   0.20 &    0.20 &     0.19 &      0.19 & 17.54 &  1332.33 &  112.99 & 18.87 &  4.46 \\
27 &  1 &  1000 &     2 & 0.18 &   0.2 &  0.17 &   0.17 &    0.17 &     0.17 &      0.16 & 17.14 &  1299.82 &   98.58 & 18.38 &  4.09 \\
27 &  1 & 10000 &     0 & 1.28 &  0.65 &  1.18 &   0.07 &    0.07 &     0.07 &      0.07 & 17.90 &  1318.52 &  101.02 & 28.09 & 47.45 \\
27 &  1 & 10000 &     1 & 0.22 &  1.26 &   NaN &   0.06 &    0.07 &     0.06 &      0.07 & 17.51 &  1314.18 &  104.27 & 23.86 & 43.75 \\
27 &  1 & 10000 &     2 & 0.54 &  0.15 &  1.87 &   0.05 &    0.05 &     0.05 &      0.05 & 15.30 &   1516.6 &  110.41 & 20.53 & 38.61 \\
27 &  3 &   100 &     0 & 0.90 &  1.17 &   NaN &   0.88 &    0.85 &     0.67 &      0.65 & 19.06 &  1248.64 &  108.72 & 26.23 &  1.09 \\
27 &  3 &   100 &     1 & 0.78 &  1.18 &   NaN &   0.73 &    0.71 &     0.57 &      0.56 & 19.11 &  1243.72 &  114.91 & 20.40 &  0.91 \\
27 &  3 &   100 &     2 & 1.03 &  1.25 &  1.22 &   0.88 &    0.87 &     0.64 &      0.66 & 18.74 &  1260.71 &  106.87 & 17.91 &  1.10 \\
27 &  3 &  1000 &     0 & 0.27 &  0.28 &  0.64 &   0.27 &    0.27 &     0.26 &      0.27 & 14.14 &  1244.38 &   102.0 & 17.38 &  4.50 \\
27 &  3 &  1000 &     1 & 0.27 &  0.27 &  0.29 &    NaN &    1.22 &     0.27 &      0.25 & 16.71 &  1230.43 &   96.04 & 18.03 &  5.00 \\
27 &  3 &  1000 &     2 & 0.23 &  0.23 &   0.3 &   0.25 &    0.26 &     0.22 &      0.24 & 17.86 &  1244.76 &  110.82 & 21.81 &  4.33 \\
27 &  3 & 10000 &     0 & 0.33 &   0.4 &  0.09 &   1.59 &    1.19 &     0.10 &      0.10 & 14.46 &  1145.31 &   93.64 & 20.00 & 42.01 \\
27 &  3 & 10000 &     1 & 0.95 &  0.36 &   1.6 &   1.73 &    1.37 &     0.10 &      0.10 & 13.35 &  1140.76 &  100.06 & 28.61 & 40.25 \\
27 &  3 & 10000 &     2 & 0.34 &  0.29 &   NaN &    NaN &    1.25 &     0.11 &      0.11 & 12.70 &  1139.38 &   92.54 & 16.04 & 41.94 \\
27 &  9 &   100 &     0 & 1.39 &     s &     s &   1.19 &    1.16 &     0.78 &      0.83 & 23.20 &        s &       s & 18.09 &  1.64 \\
27 &  9 &   100 &     1 &  NaN &     s &     s &    NaN &    1.21 &     0.81 &      0.86 & 15.52 &        s &       s & 17.38 &  1.75 \\
27 &  9 &   100 &     2 & 1.31 &     s &     s &    NaN &    1.18 &     0.81 &      0.84 & 15.42 &        s &       s & 17.15 &  1.65 \\
27 &  9 &  1000 &     0 & 0.36 &     s &     s &   0.42 &    0.47 &     0.37 &      0.39 & 12.05 &        s &       s & 14.93 &  7.01 \\
27 &  9 &  1000 &     1 & 0.38 &     s &     s &   0.40 &    0.43 &     0.38 &      0.42 & 11.80 &        s &       s & 14.86 &  7.28 \\
27 &  9 &  1000 &     2 & 0.36 &     s &     s &   0.39 &    0.42 &     0.37 &      0.40 & 12.03 &        s &       s & 14.84 &  7.25 \\
27 &  9 & 10000 &     0 & 0.24 &     s &     s &   1.29 &    1.14 &     0.16 &      0.18 & 12.46 &        s &       s & 17.29 & 57.87 \\
27 &  9 & 10000 &     1 & 0.25 &     s &     s &   0.74 &    0.78 &     0.16 &      0.18 & 12.39 &        s &       s & 17.53 & 54.68 \\
27 &  9 & 10000 &     2 & 0.72 &     s &     s &   1.15 &    1.09 &     0.16 &      0.18 & 12.40 &        s &       s & 17.04 & 55.08 \\
27 & 27 &   100 &     0 & 1.51 &     s &     s &    NaN &    1.51 &     1.15 &      1.07 & 15.08 &        s &       s & 17.46 &  3.36 \\
27 & 27 &   100 &     1 & 1.55 &     s &     s &    NaN &    1.55 &     1.20 &      1.09 & 19.93 &        s &       s & 16.76 &  3.40 \\
27 & 27 &   100 &     2 & 1.60 &     s &     s &    NaN &    1.60 &     1.21 &      1.11 & 14.94 &        s &       s & 16.46 &  3.74 \\
27 & 27 &  1000 &     0 & 0.59 &     s &     s &   0.61 &    0.64 &     0.58 &      0.62 & 11.69 &        s &       s & 15.21 & 15.43 \\
27 & 27 &  1000 &     1 & 0.59 &     s &     s &   0.61 &    0.65 &     0.57 &      0.62 & 11.72 &        s &       s & 14.92 & 14.93 \\
27 & 27 &  1000 &     2 & 0.63 &     s &     s &   0.64 &    0.68 &     0.59 &      0.64 & 11.85 &        s &       s & 14.82 & 15.17 \\
27 & 27 & 10000 &     0 & 0.33 &     s &     s &   0.88 &    0.98 &     0.23 &      0.29 & 12.75 &        s &       s & 17.66 & 77.19 \\
27 & 27 & 10000 &     1 & 0.32 &     s &     s &   1.49 &    1.27 &     0.24 &      0.28 & 12.57 &        s &       s & 17.49 & 71.97 \\
27 & 27 & 10000 &     2 & 0.42 &     s &     s &   1.53 &    1.28 &     0.23 &      0.28 & 12.91 &        s &       s & 17.70 & 70.89 \\
\bottomrule
\caption{Error (in mean $\ell_1$ distance) and time (in seconds) when computing various quantities for categorical regressions.  The MLE was computed using automatic differentiation in \texttt{jax} (and default convergence parameters). CAVI was computed using my own Python code, with a convergence criterion of a drop in the mean (over $N$) ELBO of $0.001$.  $K,M,N$ refer to the number of categories, covariates, and samples, respectively. A table entry of $s$ means that that particular inference step was skipped in order to save on computation time.  A table entry of $NaN$ means that the inference routine was unable to produce a result, and errored out.}
\label{tab:autodiff_simulations_all_results}
\end{longtable}
\normalsize 

==> inputs/fig_performance_sims_classification_expt1.tex <==
\begin{figure}[H]
\centering
\setlength{\tabcolsep}{0.01cm}  %% space between columns
\begin{tabular}{ccc}
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt1/classification_accuracy/K=3_N=18}
}
&
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt1/classification_accuracy/K=3_N=540}
} 
&
%\multirow{2}{0.16\textwidth}{}\\

\multirow{2}{0.30\textwidth}{\includegraphics[width=0.25\textwidth]{images/performance_simulations/legend}}
\\
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt1/classification_accuracy/K=30_N=1800}
}
&
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt1/classification_accuracy/K=30_N=54000}
} 
&
\\
\end{tabular}
\caption{Plotted is classification accuracy as a function of mean covariate-conditional category entropy \eqref{eqn:mean_covariate_conditional_category_entropy}, which quantifies predictability. The left column has as many samples as parameters.  The right column has $30$ times as many samples as parameters.}
\label{fig:performance_simulations_classification_accuracy_expt1}
\end{figure}


==> inputs/fig_performance_sims_classification_expt3.tex <==
\begin{figure}[H]
\centering
\setlength{\tabcolsep}{0.01cm}  %% space between columns
\begin{tabular}{ccc}
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt3/classification_accuracy/K=3_N=18}
}
&
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt3/classification_accuracy/K=3_N=1800}
} 
&
%\multirow{2}{0.16\textwidth}{}\\

\multirow{2}{0.30\textwidth}{\includegraphics[width=0.25\textwidth]{images/performance_simulations/legend}}
\\
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt3/classification_accuracy/K=30_N=1800}
}
&
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt3/classification_accuracy/K=30_N=180000}
} 
&
\\
\end{tabular}
\caption{Plotted is classification accuracy as a function of mean covariate-conditional category entropy \eqref{eqn:mean_covariate_conditional_category_entropy}, which quantifies predictability.  The left column has as many samples as parameters.  The right column has $100$ times as many samples as parameters.}
\label{fig:performance_simulations_classification_accuracy_expt3}
\end{figure}


==> inputs/fig_performance_sims_likelihood_expt1.tex <==
\begin{figure}[H]
\centering
\setlength{\tabcolsep}{0.01cm}  %% space between columns
\begin{tabular}{ccc}
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt1/likelihood/K=3_N=18}
}
&
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt1/likelihood/K=3_N=540}
} 
&
%\multirow{2}{0.16\textwidth}{}\\

\multirow{2}{0.30\textwidth}{\includegraphics[width=0.25\textwidth]{images/performance_simulations/legend}}
\\
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt1/likelihood/K=30_N=1800}
}
&
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt1/likelihood/K=30_N=54000}
} 
&
\\
\end{tabular}
\caption{Plotted is mean holdout log likelihood as a function of mean covariate-conditional category entropy \eqref{eqn:mean_covariate_conditional_category_entropy}, which quantifies predictability. The left column has as many samples as parameters.  The right column has $30$ times as many samples as parameters.  Note: some runs with the softmax MLE or baseline frequencies have holdout log likelihoods of $-\infty$.  This happens when a category that never appeared in the training set appears in the test set.}
\label{fig:performance_simulations_likelihood_expt1}
\end{figure}


==> inputs/fig_performance_sims_likelihood_expt3.tex <==
\begin{figure}[H]
\centering
\setlength{\tabcolsep}{0.01cm}  %% space between columns
\begin{tabular}{ccc}
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt3/likelihood/K=3_N=18}
}
&
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt3/likelihood/K=3_N=1800}
} 
&
%\multirow{2}{0.16\textwidth}{}\\

\multirow{2}{0.30\textwidth}{\includegraphics[width=0.25\textwidth]{images/performance_simulations/legend}}
\\
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt3/likelihood/K=30_N=1800}
}
&
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt3/likelihood/K=30_N=180000}
} 
&
\\
\end{tabular}
\caption{Plotted is mean holdout log likelihood as a function of mean covariate-conditional category entropy \eqref{eqn:mean_covariate_conditional_category_entropy}, which quantifies predictability. The left column has as many samples as parameters.  The right column has $100$ times as many samples as parameters.}
\label{fig:performance_simulations_likelihood_expt3}
\end{figure}


==> inputs/fig_performance_sims_main_body_classification.tex <==
\begin{figure}[H]
\centering
\setlength{\tabcolsep}{0.01cm}  %% space between columns
\begin{tabular}{ccc}

{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt3/classification_accuracy/K=30_N=1800}
}
&
{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt3/classification_accuracy/K=30_N=54000}
} 
& 
\includegraphics[width=0.25\textwidth]{images/performance_simulations/legend}
%\multirow{2}{0.30\textwidth}{\includegraphics[width=0.25\textwidth]{images/performance_simulations/legend}}
%\\
%{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt2/likelihood/K=3_N=1800}
%} 
%&
%{\includegraphics[width=0.5\textwidth]{images/performance_simulations/expt2/likelihood/K=30_N=180000}
%} 
%&
%\\
\end{tabular}
\caption{Plotted is classification accuracy as a function of mean covariate-conditional category entropy \eqref{eqn:mean_covariate_conditional_category_entropy}, which quantifies predictability. }
\label{fig:performance_simulations_main_body_classification}
\end{figure}


==> inputs/original_intro.tex <==

In this section, we evaluate the independent binary approximations technique in terms of computation time and estimation accuracy.    Along the way, we'd like to compare SDO to DO and variational Bayes to the MLE. 


==> inputs/original_methodology.tex <==
To proceed, we generate multiple datasets from a multi-logit (softmax) distribution with given specifications ($N$ samples, $K$ categories, $M$ covariates).   The covariates $\+X \in \R^{N \times M}$ and regression weights $\+\beta \in \R^{M \times K}$ are drawn such that all entries are taken from independent univariate Gaussians.  For a given context ($N,K,M$), we can generate different datasets by setting the random seed to a different value. 

 We then estimate the link function mapping covariates to category probabilities for a a variety of models via two different inference techniques:  
\begin{enumerate}
\item We compute the MLE, $\+\beta_{\text{MLE}}$, for a number of different models:  Diagonal Orthant Probit (DO), Simplified Diagonal Orthant Probit (SDO), Independent Binary (IB) (see Section \ref{sec:independent_binary_probit_model}), and softmax (SM) a.k.a. multi-logit.  The MLE was computed using automatic differentiation in \texttt{jax} (and default convergence parameters).  The solver used was BFGS, which is the only solver that \texttt{jax} supports\footnote{as of documentation revision 1182e7aa}. For the truly categorical models, we plug in  $\+\beta_{\text{MLE}}$ to the corresponding categorical probability formula.  For the IB model, we plug in  $\+\beta_{\text{MLE}}$ to either the DO or SDO models.  
 \item We compute CAVI for the DO and SDO models with a $\N(\+0,\+I)$ prior using the technique  described in the main body of the text.   CAVI was computed using my own Python code, with a convergence criterion of a drop in the mean (over $N,K$) ELBO of $0.01$. 
 \end{enumerate}
 
 For each method of estimating category probabilities, we then compute the distance to the ground truth category probabilities (in terms of mean $\ell1$- distance, where the mean is taken across $N$ samples).  For interpretation, a mean $\ell_1$ distance of .10 when there are $K=5$ categories  means that, on average across the $N$ samples, the entries in the category probability vector has a sum absolute deviation of $d=.10$.  This can be interpreted as the ``average" entry being off by $d/K = .02$.   Note that the minimum distance to the ground truth is 0, and the maximum distance is 2. (For example, the maximum distance for two vectors would be obtained if they were on  two different corners of the simplex for each sample, e.g. $[1,0,0, \cdots, 0]$ vs. $[0,1,0, \cdots, 0]$.  So the maximum mean distance would would be obtained if the two probability vectors being compared were on different corners of the simplex for all samples.) %A distance of 1 or lower can be easily obtained by an categorical model by just predicting the simplex center $[1/K,1/K,\cdots, 1/K]$ for all samples, regardless of covariate values. (I think - double check)



==> inputs/original_results.tex <==

In Table \ref{tab:snippet_of_autodiff_results}, we highlight the results on a few simulated datasets which typifies some patterns of interest.  

\tiny 
\begin{longtable}[H]{rrrr|rllrrrr|rllrr}
	\toprule
	\multicolumn{4}{c|}{context} & \multicolumn{7}{|c|}{error}  & \multicolumn{5}{|c|}{time (seconds)} \\
	& & & &\multicolumn{5}{|c|}{MLE} & \multicolumn{2}{|c|}{CAVI} & \multicolumn{4}{|c|}{MLE} & \multicolumn{1}{|c|}{CAVI}  \\
	 K &  M &     N &  seed &   SM &         SDO &          DO &  IB+DO &  IB+SDO &  IB+DO &  IB+SDO &    SM &      SDO &      DO &    IB &  \\
	\midrule
	      27 &
	       3 &
	    1000 &
	       0 &
	    0.27 &
	    0.28 &
	    \redbox{0.64} &
	    0.27 &
	    0.27 &
	    0.26 &
	    0.27 &
	   14.14 &
	 \redbox{1244.38} &
	   102.0 &
	   17.38 &
	     4.5 \\
    27 &
     9 &
 10000 &
     0 &
  0.24 &
  0.27 &
  0.29 &
  \redbox{1.29} &
  \redbox{1.14} &
  0.16 &
  0.18 &
 12.46 &
\redbox{1228.75} &
96.27 &
 17.29 &
 57.87 \\
	\bottomrule	
\caption{Error (in mean $\ell_1$ distance) and time (in seconds) for various inference strategies on a few highlighted datasets.  The MLE was computed using automatic differentiation in \texttt{jax} (and default convergence parameters). CAVI was computed using my own Python code, with a convergence criterion of a drop in the mean (over $N,K$) ELBO of $0.01$.  $K,M,N$ refer to the number of categories, covariates, and samples, respectively.  The results are selected from Table \ref{tab:autodiff_simulations_all_results}, with exception that some of the skipped inference steps are now computed.  A red shaded box refers to a amount of error or computation time that would presumably be considered relatively intolerable by most people. Note that the inference time for any inference technique depends on the chosen threshold; thus it could be more informative to plot error as a function of computation time.}
\label{tab:snippet_of_autodiff_results}
\end{longtable}
\normalsize 


From Table \ref{tab:snippet_of_autodiff_results}, we see 
\begin{enumerate}
\item The quality of the CAVI-IB approximation is good. We see that inference with either CAVI-IB approximation (CAVI-IB+DO or CAVI-IB+SDO) strategy produces an error which is competitive with or sometimes even better than the MLE from the true data generating process with no approximations.   
\item While producing a good approximation, the CAVI-IB strategy leads to \textit{substantially} faster and more stable results than automatic differentiation.  Computing the MLE via automatic differentiation either causes the error to blow up (notice in the second row how the error of $0.16$ blows up to between $1.1$ and $1.3$ when using MLE instead of CAVI; and in fact in some cases reported in Table \ref{tab:autodiff_simulations_all_results}, the MLE cannot even be computed at all due to computational reasons, as tensorflow returns a ``very slow compile" error), or the computation time to skyrocket (notice in the first row how the MLE for SDO gives good results, but takes 276 times longer than CAVI).  We suggest that CAVI can produce faster and/or more stable numerical results than gradient-based methods due to use of coordinate ascent. 
  \end{enumerate}
   
 \begin{remark}
Note when inspecting Table \ref{tab:snippet_of_autodiff_results} that the inference time for any inference technique depends on the chosen threshold; thus it could be more informative to plot error as a function of computation time. For example, when we set the convergence criterion of the drop in the mean (over $N,K$) ELBO to $2.0$ instead of $0.01$ for the IB-CAVI routine, the computation time drops to 11.2 seconds, and the errors change to 0.224 for IB+SDO and 0.148 for IB+DO.  	
 \end{remark}

In Table \ref{tab:autodiff_simulations_all_results},  we provide the full results. Some \textbf{observations} based on that table:

\begin{enumerate}		
\item On the IB strategy
	\begin{enumerate}
	\item The conclusions provided in the discussion of Table \ref{tab:snippet_of_autodiff_results} above still apply.
	\item For some values, the error from the IB approximation seems relatively large. See e.g. K=3, M=9, N=10000, seed=2,  where the IB approximation gives an error that is 4-6 times what would have been obtained by the MLE for softmax or SDO.   The absolute level of error relative to ground truth is perhaps still tolerable in a component wise sense - it is $\text{error}/K = .12/3 = .04$.   
	\end{enumerate}
\item On using SDO vs DO for the IB strategy 
	\begin{enumerate}
	\item As before, the \texttt{IB-SDO} error is generally systematically less than \texttt{IB-DO} error, and this is true regardless of whether we use CAVI or MLE. 
	\item However, for some regimes \texttt{IB-SDO} error appears to be systematically \textit{greater} than \texttt{IB-DO}.  See the rows where $K=27, M=27$. 
		
		\begin{task}
		With large $K$ and $M$, DO might be doing better not because of size per se, but because in those scenarios, no category dominates the probability.  Investigate whether this is happening, and rerun some of the larger runs with sparsity in the data generating process.
		\end{task}

	\item We have expressed concerns earlier that comparisons between SDO and DO may be warped by the fact that the same prior $\N(\+0,\+I)$ may have different implications in each case.   The experiment here is able to dispel those concerns, as the relationship between \texttt{CAVI-IB+SDO} and \texttt{CAVI-IB+DO} tends to mimic the relationship between \texttt{MLE-IB+SDO} and \texttt{MLE-IB+DO}. 
	%\item 
%		\begin{question}
%		We see cases where IB-MLE+(S)DO has much larger error than (S)DO-MLE even when $N$ is large.  For example, see K=3, M=27, N=10000, seed=1, where the error compared to ground truth is given by: IB MLE + SDO: 0.131, IB MLE + DO: 0.178,  SDO MLE: 0.055, DO MLE: 0.285.  Doesn't this suggest that Johndrow et al. (2013) were wrong that the IB beta is an MLE for the DO/SDO model?!?!!	
%	 \end{question}

	\end{enumerate}
\item On VB estimates vs. MLE estimates 
	\begin{enumerate}
	\item When $N$ is sufficiently small relative to $K,M$, \texttt{IB-CAVI+(S)DO} can beat \texttt{IB-MLE+(S)DO} -- in fact, it can even  closer to ground truth than even the softmax MLE.
	\item In many cases, \texttt{IB-CAVI + (S)DO} tends to concentrate around \texttt{IB-MLE+(S)DO} -- the errors converge as N gets large.
	\item \textit{However}, for some large settings, AD returns junk for everything, compared to the CAVI code. See, for instance, $K=9, N=10000, M=27, seed=2$.  Is this a function of the Bayesian approach or the numerical implementation?  I think the latter is more likely since we're not exactly in a "small-data" scenario (the number of samples $N=10,000$ is still about $40x$ larger than the number of parameters, $KM=243$).
	\item The way that AD tends to produce junk differs between SDO and DO.  For computing the DO-MLE, tensorflow tends to returns a ``very slow compile" error after a short amount of time, yielding relatively quick inference but with large error.  For the SDO-MLE, tensorflow tends to produce results that can be of high quality, but take an exceedingly long time to produce. 
	\item Finally, some discussions, conjectures, and questions:

	\begin{discussion}
	Any thoughts or recommendations on how the numerical optimization was done?
	\end{discussion}
	
	\begin{question}
	How is the \texttt{AD} library differentiating through $\Phi$ in the first place?	
	\end{question}
	 
	 \begin{conjecture}
	One possible advantage of CAVI even over the MLE - CAVI does not require explicitly differentiating through the Gaussian cdf $\Phi$.
	 \end{conjecture} 
	\end{enumerate}
\end{enumerate}
